Better Teacher Better Student: Dynamic Prior Knowledge for Knowledge Distillation

Knowledge distillation (KD) has shown very promising capabilities in transferring learning representations from large models (teachers) to small models (students). However, as the capacity gap between students and teachers becomes larger, existing KD methods fail to achieve better results. Our work shows that the `prior knowledge' is vital to KD, especially when applying large teachers. Particularly, we propose the dynamic prior knowledge (DPK), which integrates part of teacher's features as the prior knowledge before the feature distillation. This means that our method also takes the teacher's feature as `input', not just `target'. Besides, we dynamically adjust the ratio of the prior knowledge during the training phase according to the feature gap, thus guiding the student in an appropriate difficulty. To evaluate the proposed method, we conduct extensive experiments on two image classification benchmarks (i.e. CIFAR100 and ImageNet) and an object detection benchmark (i.e. MS COCO. The results demonstrate the superiority of our method in performance under varying settings. Besides, our DPK makes the performance of the student model positively correlated with that of the teacher model, which means that we can further boost the accuracy of students by applying larger teachers. More importantly, DPK provides a fast solution in teacher model selection for any given model.

==> sections/checklist.tex <==
\newpage
\section*{Checklist}

\begin{enumerate}
\item For all authors...
\begin{enumerate}
\item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
\answerYes{}

\item Did you describe the limitations of your work?
\answerYes{In the supplementary material.}
\item Did you discuss any potential negative societal impacts of your work?
\answerYes{In the supplementary material.}
\item Have you read the ethics review guidelines and ensured that your paper conforms to them?
\answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA
        \item Did you include complete proofs of all theoretical results?
    \answerNA
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
\item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
\answerNA

\item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
\answerYes{In the supplementary material.}
\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
\answerNA

\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
\answerYes{In the supplementary material.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
\item If your work uses existing assets, did you cite the creators?
\answerNA

\item Did you mention the license of the assets?
\answerNA

\item Did you include any new assets either in the supplemental material or as a URL?
\answerNA

\item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
\answerNA

\item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
\answerNA
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
\item Did you include the full text of instructions given to participants and screenshots, if applicable?
\answerNA

\item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
\answerNA

\item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
\answerNA
\end{enumerate}
\end{enumerate}

==> tables/ablation_multi_stage.tex <==
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{1.0mm}{
\begin{tabular}{lc|ccc}
\toprule
Teacher & Acc. & \small{Stage 4} & \small{Stage 3\&4} & \small{Stage 2\&3\&4}  \\
\toprule
\multirow{2}{*}{ResNet34} & Top-1 &{\color{mygray}72.46} & \textbf{72.51} & {\color{mygray}72.45} \\
& Top-5  &{\color{mygray}90.67} & \textbf{90.77} &{\color{mygray}90.55} \\
\midrule
\multirow{2}{*}{ResNet50} & Top-1  &{\color{mygray}72.65} & \textbf{72.87} &{\color{mygray}72.82} \\
& Top-5  &{\color{mygray}90.65} & \textbf{90.92} &{\color{mygray}90.83} \\
\midrule
\multirow{2}{*}{ResNet101} & Top-1  &{\color{mygray}72.87} & {\color{mygray}72.99} &\textbf{73.00} \\
& Top-5  &{\color{mygray}90.96} &{\color{mygray}90.94} & \textbf{91.03} \\
\midrule
\multirow{2}{*}{ResNet152} & Top-1  &{\color{mygray}72.74} &\textbf{73.29} & {\color{mygray}73.09} \\
& Top-5  &{\color{mygray}90.91} & \textbf{91.10} &{\color{mygray}90.95} \\
\bottomrule
\end{tabular}}}
\caption{{\bf Ablations on multi-stage distillation.} We adopt ResNet18 as student model.}
\label{tb:mutli_stage}

==> tables/different_teacher.tex <==
% \begin{table}[]
\centering
\renewcommand\arraystretch{1.0}
\setlength{\tabcolsep}{0.5mm}{
\small
\begin{tabular}{cc|cccc}
\toprule
                                               & \multirow{2}{*}{Model Name} & \multicolumn{4}{c}{Accuracy (\%)} \\
                                               &                         & Top-1  & Top-5  & Top-1  & Top-5  \\ \midrule
\multicolumn{1}{c|}{Student}                   & R18                & --     & --     & 69.55  & 89.09  \\ \midrule
\multicolumn{1}{c|}{\multirow{8}{*}{Teachers}} & R34\_KD     & 75.81  & 92.70  & 71.60  & 90.19  \\
\multicolumn{1}{c|}{}                          & R50\_KD     & 75.86  & 92.88  & 71.63  & 90.16  \\
\multicolumn{1}{c|}{}                          & R101\_KD    & 75.97  & 92.73  & 71.32  & 89.95 \\
\multicolumn{1}{c|}{}                          & R152\_KD    & 76.24  & 92.80  & 71.21  & 89.89  \\ \cmidrule{2-6} 
\multicolumn{1}{c|}{}                          & R34\_AT     & 75.81  & 92.70  & 70.58  & 89.76  \\
\multicolumn{1}{c|}{}                          & R50\_AT     & 75.86  & 92.88  & 70.10  & 89.58  \\
\multicolumn{1}{c|}{}                          & R101\_AT    & 75.97  & 92.73  & 70.57  & 89.64 \\
\multicolumn{1}{c|}{}                          & R152\_AT    & 76.24  & 92.85  & 70.39  & 89.55 \\ \bottomrule
\end{tabular}}
\caption{Same performance, different teachers.}
% \end{table}



==> tables/main_results_cifar_100_heterogeneous.tex <==
\begin{table}[!hbpt]
\caption{Top-1 accuracy (\%) comparison of various KD methods across \textit{heterogeneous} teacher-student pairs on CIFAR-100. ``N/A'' indicates results are not available and best results are marked in bold.}
\renewcommand\arraystretch{0.6}
\setlength{\tabcolsep}{0.50mm}{
\small
\begin{tabular}{c|rcccccc}
\toprule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Distillation\\ Mechanism\end{tabular}} & Teacher  & VGG13       & ResNet50    & ResNet50 & ResNet32$\times$4 & ResNet32$\times$4 & WRN40-2      \\
                                                                                  & Acc.     & 74.64       & 79.34       & 79.34    & 79.42             & 79.42             & 79.42        \\ \cmidrule{2-8} 
                                                                                  & Student  & MobileNetV2 & MobileNetV2 & VGG8     & ShuffleNetV1      & ShuffleNetV2      & ShuffleNetV1 \\
                                                                                  & Acc.     & 64.60       & 64.60       & 70.36    & 70.50             & 71.82             & 70.50        \\ \midrule


\multirow{2}{*}{Logits}                                                           & KD~\cite{Hinton2015DistillingTK}       & 67.37   & 67.35   & 73.81   & 74.07     & 74.45     & 74.83    \\
                                                                                  & DKD~\cite{zhao2022dkd}                 & 69.71   & 70.35   & N/A     & 76.45     & 77.07     & 76.70     \\ \midrule

\multirow{12}{*}{Features}                                                        & FitNets~\cite{Romero2015FitNetsHF}      & 64.14   & 63.16    & 70.69    & 73.59     & 73.54    & 73.73    \\

                                                                                  & FT~\cite{kim2018paraphrasing}           & 61.78   & 60.99    & 70.29    & 71.75     & 72.50    & 72.03    \\
                                                                                  & NST~\cite{huang2017like}                & 58.16   & 64.96    & 71.28    & 74.12     & 74.68    & 74.89    \\
																				  & AT~\cite{Zagoruyko2017PayingMA}         & 59.40   & 58.58    & 71.84    & 71.73     & 72.73    & 73.32    \\
																			      & PKT~\cite{Passalis2018LearningDR}       & 67.13   & 66.52    & 73.01    & 74.10     & 74.69    & 73.89    \\
																			      & SP~\cite{Tung2019SimilarityPreservingKD}& 66.30   & 68.08    & 73.34    & 73.48     & 74.56    & 74.52    \\
                                                                                  & CC~\cite{peng2019correlation}          & 64.86   & 65.43   & 70.25    & 71.14     & 71.29     & 71.38     \\
                                                                                  & RKD~\cite{Park2019RelationalKD}        & 64.52   & 64.43   & 71.50    & 72.28     & 73.21     & 72.21     \\
                                                                                  & VID~\cite{Sungsoo19Variational}        & 65.56   & 67.57   & 70.30    & 73.38     & 73.40     & 73.61     \\
                                                                                  & CRD~\cite{Tian2020ContrastiveRD}       & 69.73   & 69.11   & 74.30    & 75.11     & 75.65     & 76.05     \\
                                                                                  % & ICKD-C~\cite{liu2021exploring}         & 75.57   & 74.63   & 71.69    & 71.91     & 74.11     & 75.48     \\
                                                                                  & OFD~\cite{heo2019comprehensive}        & 69.48   & 69.04   & N/A      & 75.98     & 76.82     & 75.85    \\
                                                                                  & ReviewKD~\cite{chen2021reviewkd}       & 70.37   & 69.89   & N/A      & 77.45     & 77.78     & 77.14     \\ \cmidrule{2-8} 
                                                                                  & \textbf{MFD}    & 68.98  & 69.22 & \textbf{74.92} & 74.82 & 76.19 & 75.89           \\ \bottomrule
\end{tabular}}
\label{tb:heterogeneous}
\end{table}

==> tables/results.tex <==

\begin{figure*}[!hbpt]
\vspace{-0.cm}
\begin{minipage}[t]{.48\linewidth}
\setlength{\tabcolsep}{3.pt}
\captionof{table}{Results when using longer burn-in phase on CIFAR-10 (i.e., running the burn-in phase for 100 epochs, compared to 40 epochs in Table~\ref{table2}).}
\vspace{-0.3cm}
  \begin{center}
  \renewcommand*{\arraystretch}{1.}
  %\begin{sc}
    \begin{tabular}{l|c|cccc}
    \toprule
\multirow{2}{*}{Method}    & Loss & No &  \multicolumn{3}{c}{$\ell_{\infty}$-norm clip bound}   \\
    & scaling & clip & 10 & 1 & 0.1  \\
    \midrule
& 1 &  89.34 & 89.34 & 89.91 & 89.99 \\
 Poisoned & 10 &  45.29 & 84.45 & 89.91 & 89.99 \\
 trigger & 20 &  16.62 & 84.45 & 89.91 & 89.99 \\
 & 50 &  10.24 & 84.45 & 89.91 & 89.99 \\
 \midrule
  & 0.01 & 80.35 & 80.35 &  80.35 & 83.32 \\
 {\textbf{Accu.}} & 0.02 &  25.45 & 25.45 & 25.45 & 76.06 \\
 {\textbf{phase}} & 0.05 & 12.03 & 12.03&  15.53 & 70.00 \\
 & 0.08 & 11.07  &11.07   &14.23  & 64.74 \\
    \bottomrule
    \end{tabular}%
    \vspace{-0.cm}
    \label{table31}
 % \end{sc}
  \end{center}
  \end{minipage}
  \hspace{0.45cm}
\begin{minipage}[t]{.48\linewidth}
\setlength{\tabcolsep}{3.pt}
\captionof{table}{Classification accuracy (\%) on MNIST after the model updating by the trigger batch. The accumulative phase runs for 200 steps ($\frac{1}{3}$ epochs), with perturbation constraint $\epsilon=16/255$ and step size $\alpha=2/255$.}
\vspace{-0.3cm}
  \begin{center}
  \renewcommand*{\arraystretch}{1.}
  %\begin{sc}
    \begin{tabular}{c|c|cccc}
    \toprule
\multirow{2}{*}{Method}    & Loss & No &  \multicolumn{3}{c}{$\ell_{\infty}$-norm clip bound}   \\
    & scaling & clip & 10 & 1 & 0.1  \\
    \midrule
& 1 &  98.27 & 98.27 & 98.27 & 98.28 \\
 Poisoned & 10 &  95.49 & 95.49 & 98.12 & 98.28 \\
 trigger & 20 &  84.09 & 89.24 & 98.12 & 98.28 \\
 & 50 &  31.93 & 89.24 & 98.12 & 98.28 \\
 \midrule
 {\textbf{Accu.}} & \multirow{2}{*}{0.08} &  \multirow{2}{*}{22.49} & \multirow{2}{*}{22.49} & \multirow{2}{*}{32.87} & \multirow{2}{*}{51.28} \\
 {\textbf{phase}} &  &  &  &   &  \\
    \bottomrule
    \end{tabular}%
    \vspace{-0.cm}
    \label{table32}
 % \end{sc}
  \end{center}
\end{minipage}
  \vspace{-0.5cm}
  \end{figure*}



==> tables/same_teacher.tex <==
% \begin{table}[]
\renewcommand\arraystretch{1.0}
\setlength{\tabcolsep}{0.5mm}{
\small
\begin{tabular}{cc|cccc}
\toprule
                                               & \multirow{2}{*}{Model Name} & \multicolumn{4}{c}{Accuracy (\%)} \\
                                               &                         & Top-1  & Top-5  & Top-1  & Top-5  \\ \midrule
\multicolumn{1}{c|}{Student}                   & R18                & --     & --     & 69.55  & 89.09  \\ \midrule
\multicolumn{1}{c|}{\multirow{8}{*}{Teachers}} & R34\_KD\_v1     & 73.31  & 91.42  & 70.68  & 90.16  \\
\multicolumn{1}{c|}{}                          & R34\_KD\_v2     & 74.37  & 91.90  & 71.36  & 90.08  \\
\multicolumn{1}{c|}{}                          & R34\_KD\_v3     & 75.81  & 92.70  & 71.60  & 90.19  \\
\multicolumn{1}{c|}{}                          & R34\_KD\_v4     & 76.27  & 92.96  & 71.41  & 90.22  \\ \cmidrule{2-6} 
\multicolumn{1}{c|}{}                          & R34\_AT\_v1     & 73.31  & 91.42  & 70.59  & 89.73  \\
\multicolumn{1}{c|}{}                          & R34\_AT\_v2     & 74.32  & 91.91  & 70.35  & 89.61  \\
\multicolumn{1}{c|}{}                          & R34\_AT\_v3     & 75.81  & 92.70  & 70.58  & 89.76  \\
\multicolumn{1}{c|}{}                          & R34\_AT\_v4     & 76.27  & 92.26  & 70.45  & 89.74  \\ \bottomrule
\end{tabular}}
\caption{Same teacher, varying performances}
% \end{table}
